qPMS Sigma -- An Efficient and Exact Parallel Algorithm for the Planted $(l, d)$ Motif Search Problem

Motif finding is an important step for the detection of rare events occurring in a set of DNA or protein sequences. Extraction of information about these rare events can lead to new biological discoveries. Motifs are some important patterns that have numerous applications including the identification of transcription factors and their binding sites, composite regulatory patterns, similarity between families of proteins, etc. Although several flavors of motif searching algorithms have been studied in the literature, we study the version known as $ (l, d) $-motif search or Planted Motif Search (PMS). In PMS, given two integers $ l $, $ d $ and $ n $ input sequences we try to find all the patterns of length $ l $ that appear in each of the $ n $ input sequences with at most $ d $ mismatches. We also discuss the quorum version of PMS in our work that finds motifs that are not planted in all the input sequences but at least in $ q $ of the sequences. Our algorithm is mainly based on the algorithms qPMSPrune, qPMS7, TraverStringRef and PMS8. We introduce some techniques to compress the input strings and make faster comparison between strings with bitwise operations. Our algorithm performs a little better than the existing exact algorithms to solve the qPMS problem in DNA sequence. We have also proposed an idea for parallel implementation of our algorithm.

==> algorithms.tex <==
\chapter{Algorithms}\label{ch:algorithms}

\section{Sample Algorithm}
In Algorithm~\ref{alg1} we show how to calcute $y=x^n$.

\begin{algorithm}
  \caption{Calculate $y = x^n$}
  \label{alg1}
  \begin{algorithmic}
    \input{algorithms/yxn.alg}
  \end{algorithmic}
\end{algorithm}

\endinput


==> buetcseugthesisabstract.tex <==
% Do not change these lines
\renewcommand{\abstractname}{\textbf{{\Large ABSTRACT}}}
\addcontentsline{toc}{chapter}{\textbf{\normalsize{\emph{ABSTRACT}}}}

% You need to change the text for abstract
\begin{abstract}\thispagestyle{plain}
Motif finding is an important step for the detection of rare events occurring in a set of DNA or protein sequences. Extraction of information about these rare events can lead to new biological discoveries. Motifs are some important patterns that have numerous applications including the identification of transcription factors and their binding sites, composite regulatory patterns, similarity between families of proteins, etc. Although several flavors of motif searching algorithms have been studied in the literature, we study the version known as $ (l, d) $-motif search or Planted Motif Search (PMS). In PMS, given two integers $ l $, $ d $ and $ n $ input sequences we try to find all the patterns of length $ l $ that appear in each of the $ n $ input sequences with at most $ d $ mismatches. We also discuss the quorum version of PMS in our work that finds motifs that are not planted in all the input sequences but at least in $ q $ of the sequences. Our algorithm is mainly based on the algorithms qPMSPrune, qPMS7, TraverStringRef and PMS8. We introduce some techniques to compress the input strings and make faster comparison between strings with bitwise operations. Our algorithm performs a little better than the existing exact algorithms to solve the qPMS problem in DNA sequence. We have also proposed an idea for parallel implementation of our algorithm.

\end{abstract}

\endinput


==> buetcseugthesisacknowledgement.tex <==
% Do not chage this part
\begin{center}
  \textbf{{\Large ACKNOWLEDGEMENT}}\\[60pt]
\end{center}
\addcontentsline{toc}{chapter}{\textbf{\normalsize{\emph{ACKNOWLEDGEMENT}}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The text herein are only samples, change them to your taste
First and foremost we would like to offer our deepest gratitude to our supervisor, Professor Dr.\ Md.\ Abul Kashem Mia for introducing us to the fascinating world of bioinformatics, supporting us throughout the full session of our thesis with his patience and knowledge. He shared his wisdom with us in analyzing subject matters, valued our thinking approach to synthesize those topics and encouraged us at the time of disappointment. His invaluable guidance, deep insights and suggestions drove us towards better ways of thinking about the problem. One simply could not wish for a better or friendlier supervisor.  

We would like to sincerely thank Md. Arifuzzaman and Md. Shazibul Islam Shamim, who have previously worked in this particular field and shared the primitive study materials and gave effective guidelines whenever we needed. The level of patience and time given by them is really praiseworthy.

Finally, we want to dedicate the essence of our purest respect to our parents who have made our existences possible. They always believed in us even at the moment when we were losing our believes in ourselves. It is not really we who reached here but of course it is our kind parents who gave us hope and inspiration.

\vspace*{20.0mm}

\begin{minipage}[t]{0.2\textwidth}
  Dhaka\par
  \thesisdate
\end{minipage}%
\hfill
\begin{minipage}[t]{0.45\textwidth}
  \begin{enumerate}
    \vspace{-0.75\baselineskip}
    \DTLforeach{ThesisStudents}{\StudentName=Column1}{\item[]\StudentName}
  \end{enumerate}
\end{minipage}

\endinput


==> chapterwithmathintitle.tex <==
\chapter{$k$-safe Labeling of Petersen Graph}\label{safeklabelingpetersen}

In 1898, Petersen produced a trivalent graph with no leaves, now
called the Petersen graph~\cite{holton1993petersen}.  In this chapter
we study $k$-safe labeling for the Petersen graph. We also give upper
bound for the span of the Petersen graph. We provide necessary proof
for the upper bound.

\endinput



==> citeexamples.tex <==
\chapter{Citation Examples}\label{ch:citations}

In this chapter we show how we can cite the references.


\section{See the Citations}
\label{sec:cite}

As discussed by authors 
in~\cite{das2007survey,nicolae2014efficient,nicolae2015qpms9} we can
further show how this affects
us. Moreover~\cite{tanaka2014improved,gohardaninew,huan2015efficient}
can be examples for the previous works. Among
these~\cite{aickelin2005artificial,faruque2016modelling,durocher2015graphs,rahman2016absent,hashem2013countering,farhad2016mapping,dinh2012qpms7}
are the prominent ones. Also you can take a look
at~\cite{jones2004introduction,xiao2016qpms10}.


\endinput





==> indexcreation.tex <==
\chapter{Index Creation}
\section{BUET}
Bangladesh University of Engineering and Technology, abbreviated as
BUET\index{BUET}, is one of the most prestigious institutions for
higher studies in the country. About 5500 students are pursuing
undergraduate\index{BUET!undergraduate} and
postgraduate\index{BUET!postgraduate} studies in engineering,
architecture, planning and science in this institution. At present,
BUET has sixteen teaching departments under five faculties and it has
three institutes. Every year the intake of undergraduate students is
around 900, while the intake of graduate students in Master's and PhD
programs is around 1000. A total of about five hundred teachers are
teaching in these departments and institutes. There are additional
teaching posts like Dr.\ Rashid Professor, Professor Emeritus and
Supernumerary Professors.
 
\section{Campus}
The BUET campus is in the heart of Dhaka\index{Dhaka} --- the capital
city of Bangladesh. It has a compact campus with halls of residence
within walking distances of the academic buildings. The physical
expansion of the University over the last three decades has been
impressive with construction of new academic buildings,
auditorium\index{BUET!auditorium} complex, halls of residence, etc.
 
\section{History}\index{BUET!History}
BUET is the oldest institution for the study of Engineering and
Architecture in Bangladesh. The history of this institution dates back
to the days of Dhaka Survey School which was established at
Nalgola\index{Nalgola}, in Old Dhaka in 1876 to train Surveyors for
the then Government of Bengal of British India. As the years passed,
the Survey School became the Ahsanullah School of
Engineering\index{Ahsanullah School of Engineering} offering
three-year diploma courses in Civil, Electrical and Mechanical
Engineering. In recognition of the generous financial contribution
from the then Nawab of Dhaka, it was named after his father Khawja
Ahsanullah. It moved to its present premises in 1912. In 1947, the
School was upgraded to Ahsanullah Engineering College as a Faculty of
Engineering under the University of Dhaka, offering four-year
bachelor’s courses in Civil, Electrical, Mechanical, Chemical and
Metallurgical Engineering. In order to create facilities for
postgraduate studies and research, Ahsanullah Engineering College was
upgraded to the status of a University in 1962 and was named East
Pakistan University of Engineering and Technology. After the War of
Liberation in 1971\index{1971|see {War of Liberation}}\index{War of
  Liberation}, Bangladesh became an independent state and the
university was renamed as the Bangladesh University of Engineering and
Technology.
 
\section{Students}
Till today, it has produced around 25,000 graduates in different
branches of engineering and architecture, and has established a good
reputation all over the world for the quality of its graduates, many
of whom have excelled in their profession in different parts of the
globe. It was able to attract students from countries like
India\index{India}, Nepal\index{Nepal}, Iran\index{Iran},
Jordan\index{Jordan}, Malaysia\index{Malaysia}, Sri Lanka\index{Sri
  Lanka}, Pakistan\index{Pakistan} and Palestine\index{Palestine}.
 
\section{Departments}
Both Undergraduate and Postgraduate studies and research are now among
the primary functions of the University. Eleven departments under five
faculties offer Bachelor Degrees, while most of the departments and
institutes offer Master's Degrees and some of the departments have
Ph.D. programs. In addition to its own research programs, the
university undertakes research programs sponsored by outside
organizations like European Union, UNO,
Commonwealth\index{Commonwealth}, UGC\index{UGC}, etc. The expertise
of the University teachers and the laboratory facilities of the
University are also utilized to solve problems and to provide
up-to-date engineering and technological knowledge to the various
organizations of the country.


\endinput

==> introduction2.tex <==
\chapter{Introduction}\label{intro}
(incomplete)
In this chapter we briefly discuss about motifs,
what are they and why are we interested in them. 


\section{What are Motifs}
Motif\index{Motif} usually means a pattern. For any sequence
of objects to be called a pattern, it has to have at least
more than one instance. To define more precisely, a motif
should have significantly higher occurrence in a given array
or list compared to what you would obtain in a randomized
array of same components. Here array means an arranged set
such as a genome or a protein structure. Genome is an array
of nucleotides and protein structure is an array of amino acids.



\subsection{Sequence Motifs}
By sequence motif\index{Motif!Sequence Motif} we mean a pattern
of nucleotide or amino acid that has specific biological
significance. In other words, they are pattern of a DNA array or
protein sequence. They may be also called regulatory sequence
motifs. This kind of motifs are commonly studied in bioinformatics.
They are becoming increasingly important in the analysis of gene
regulation. In our thesis we will only discuss about this type of motifs.


\subsection{Structural Motifs}
Structural motifs\index{Motif!Structural Motif} are a super-secondary
structure in a chain like biological molecules such as protein.
It is formed by three dimensional alignment of amino acids
which may not be adjacent. 


\section{Regulatory Motifs in DNA}
Regulatory motifs\index{Regulatory Motifs} are some short nucleotide
sequence that regulates the expression of genes such as controlling
the situations under which the genes will be turned on or off.
For example:~\cite{jones2004introduction} Fruit flies have a small
set of \textit{immunity genes} that are dormant
in their genome. But when its organisms get infected somehow the genes
got switched on. It turns out that many immunity genes in
the fruit fly genome have strings that are reminiscent of TCGGGGATTTCC,
located upstream of the genes start. This string are called $ _{NF-\kappa}$B
binding sites which are important examples of regulatory motifs. Proteins
known as \textit{transcription factors} bind to these motifs, encouraging
RNA polymerase to transcribe the downstream genes.


\subsection{Regulatory Regions}
As discussed in~\cite{Riethoven2010} regulation of gene expression
is an essential part of every organism. Certain regions,
called cis-regulatory elements, on the DNA are footprints for
the trans-acting proteins involved in transcription. DNA
regions involved in transcription and transcriptional regulation
are called regulatory regions (RR).\index{Regulatory Motifs!Regulatory Regions}
Every gene contains a RR typically
stretching 100-1000 bp upstream of the transcriptional start site.
In  \Cref{fig:rr} we see the structure of a eukaryotic protein
coding gene. Regulatory sequence controls when and where expression
occurs for the protein coding region (red). Promoter and enhancer
regions (yellow) regulate the transcription of the gene into a
pre-mRNA which is modified to remove introns (light grey) and
add a 5' cap and ploy-A tail (dark grey). The mRNA 5' and 3'
untranslated regions (blue) regulate translation into the
final protein product.


\begin{figure}[!tb]
	\centering
	\includegraphics[width=0.9\textwidth]{figures/rr}
	\caption{The structure of a eukaryotic protein-coding gene.}
	\label{fig:rr}
\end{figure}


\subsection{Transcription Factor Binding Sites}
\index{Regulatory Motifs!Transcription Factor Binding Sites}
A transcription factor (TF) is a protein that can bind to DNA
and regulate gene expression. The region of the gene to which
TF binds is called a transcription factor binding site (TFBS).
TFs influence gene expression by binding to a specific location
in the respective gene’s regulatory region which is known as
TFBSs or motifs.~\cite{wei2007comparative} TFBS can be located
anywhere within the RR. TFBS may vary slightly across different
regulatory regions since non-essential bases could mutate.
TFBSs are a part of either the promoter or enhancer region of a gene.
A promoter sits upstream and contains three important regions-
the regulatory protein binding site, the transcription factor
binding site, and the RNA polymerase binding site.
In \Cref{fig:tfbs} we see a picture of promoter
and enhancer. An enhancer is usually far upstream of a gene.

\begin{figure}[!tb]
	\centering
	\includegraphics[width=0.9\textwidth]{figures/tfbs}
	\caption{Transcription Factor Binding Sites.}
	\label{fig:tfbs}
\end{figure}


\section{Motifs Logos}
Motifs can mutate at the non important bases. Motif logo\index{Motifs!Motifs Logos}
is one type of representation of the variable and fixed regions of
the motif. 


\section{Problem Description}
\section{Review of Literature}
\section{Why Study Motifs}


\endinput

%See these examples:
%\begin{itemize}
%	\item 
%	\item \Cref{fig:sample} is a sample figure.
%	\item \Cref{tab_our} is a table.
%	\item \Cref{sec:cite} in \Cref{ch:citations} shows some examples of
%	  citations.
%\end{itemize}

%\section{How to Write a Section}
%
%This is for writing section.
%
%\section{How to Add Table and Figures}\label{contribution}
%You should refer a figure as, ``\Cref{fig:sample} is a sample
%figure''.
%
%\begin{figure}[!tb]
%  \centering
%  \includegraphics[width=0.9\textwidth]{figures/sample}
%  \caption{This is a sample figure.}
%  \label{fig:sample}
%\end{figure}
%
%				
%Then we applied same test cases to our modified algorithm i.e.\ the
%heuristic algorithm with our new operation \textit{Block Reversal}. The
%performance is shown in \Cref{tab_our}.


%\begin{table}[!tb]
%	\begin{center}
%		\caption{Degenerate nucleotide code}
%		\label{tab_nucleotide_code}
%		
%		\begin{tabular}{|l|r|r|r|}
%			
%			\hline
%			IUB	& Nucleotides	& Name	& [pA,pc,pG,pT]\\	
%			\hline
%			
%			A 	& A & Adenine & $ [1, 0, 0, 0] $ \\
%			C	&C	&Cytosine	&$ [0, 1, 0, 0] $\\
%			
%			G	&G	&Glutamine	 &$[0, 0, 1, 0] $\\
%			
%			T	&T	&Tyrosine	&$ [0, 0, 0, 1] $\\
%			
%			S	&C or G		&Strong		&$ [0, \frac{1}{2}, \frac{1}{2}, 0] $\\
%			
%			W	&A or T		&Weak	&$ [\frac{1}{2}, 0, 0, \frac{1}{2}] $\\
%			
%			R	&A or G	&PuRine		&$ [\frac{1}{2}, 0, \frac{1}{2}, 0] $\\
%			
%			Y	&C or T	&pYrimidine		&$ [0, \frac{1}{2}, 0, \frac{1}{2}] $\\
%			
%			M	&A or C	&aMino group	&$ [\frac{1}{2}, \frac{1}{2}, 0, 0] $\\
%			
%			K	&G or T		&Keto group		&$ [0, 0, \frac{1}{2}, \frac{1}{2}] $\\
%			
%			B	&C or G or T		&Not A	&$ [0, \frac{1}{3}, \frac{1}{3}, \frac{1}{3}] $\\
%			
%			D	&A or G or T	&Not C	&$ [\frac{1}{3}, 0, \frac{1}{3},\frac{1}{3}] $\\
%			
%			H	&A or C or T  &Not G  &$ [\frac{1}{3}, \frac{1}{3}, 0, \frac{1}{3}] $\\
%			
%			V	&A or C or G 	&Not T &$ [\frac{1}{3}, \frac{1}{3}, \frac{1}{3}, 0] $\\
%			
%			N	&A, C, G or T 	&aNy base &$ [\frac{1}{4}, \frac{1}{4},\frac{1}{4},\frac{1}{4}] $\\
%			\hline
%		\end{tabular}
%	\end{center}
%	
%\end{table}


%\begin{table}[!tb]
%  \begin{center}
%    \caption{Performance table of \emph{Block reversal} in a heuristic algorithm ($n=20$)}
%    \label{tab_our}
%
%    \begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|r|}
%      \hline
%      $\alpha$     & $\alpha n$ & \multicolumn{11}{c|}{Test Cases} & \multicolumn{1}{c|}{Average \# of}                                     \\
%      \cline{3-13} &            & 1                                & 2  & 3  & 4  & 5  & 6  & 7  & 8  & 9  & 10 & 11 & calculated operation \\
%      \hline
%      0.1        & 2          & 2                                & 2	& 2  & 2  & 2  & 2  & 2  & 2  &	2  & 2	& 2  & 2                    \\
%      0.2        & 4          & 4                                & 4	& 5  & 2  & 4  & 4  & 4  & 4  &	2  & 4	& 4  & 3.73                 \\
%      0.3        & 6          & 5                                & 6	& 6  & 6  & 6  & 7  & 6  & 5  &	6  & 6	& 6  & 5.91                 \\
%      0.4        & 8          & 7                                & 8	& 5  & 6  & 7  & 6  & 6  & 7  &	8  & 8	& 7  & 6.82                 \\
%      0.5        & 10         & 9                                & 10	& 6  & 12 & 10 & 8  & 10 & 10 &	7  & 7	& 10 & 9                    \\
%      0.6        & 12         & 9                                & 12	& 16 & 10 & 12 & 12 & 9  & 11 &	12 & 9	& 12 & 11.27                \\
%      0.7        & 14         & 13                               & 7	& 18 & 15 & 14 & 8  & 13 & 11 &	13 & 13	& 14 & 12.64                \\
%      0.8        & 16         & 10                               & 17	& 14 & 16 & 13 & 16 & 13 & 11 &	13 & 17	& 13 & 13.91                \\
%      0.9        & 18         & 14                               & 16	& 15 & 12 & 15 & 11 & 15 & 11 &	15 & 12	& 12 & 13.45                \\
%      1          & 20         & 18                               & 11	& 13 & 11 & 13 & 15 & 17 & 17 &	13 & 18	& 12 & 14.36                \\
%      \hline
%    \end{tabular}
%  \end{center}
%\end{table}
%



==> motiffindingproblem.tex <==
\chapter{To The Motif Finding Problem}\label{motiffindingproblem}
Our target is to identify a motif from a DNA sequence. In our study
we only deal with transcription factor binding sites. We will give
the formal definition of the motif finding problem later. Assume
that we are given some DNA sequence of nucleotides which are generated
randomly. Now, we want to find a secret pattern that occurs at least
one time in every given DNA sequence without any prior knowledge
about how it looks like. This pattern is our motif.

Some complications encountered while finding motifs:
\begin{itemize}
	\item We do not know the motif sequence.
	\item Hence we donot know what to search for in the DNA sequence.
	\item We do not know where the motifs are located relative to
	the starting index of the sequence.
	\item Motifs can differ in one or more positions in their
	sequence which is called mutations.
	\item How to discern functional motifs from random ones?
	
\end{itemize}

The idea is illustrated in the \Cref{fig:seq1}, \Cref{fig:seq2}
and \Cref{fig:seq2}.

\begin{figure}%[!tb]
	\centering
	\includegraphics[width=0.6\textwidth]{figures/seq1}
	\caption{Seven random sequences.}
	\label{fig:seq1}
\end{figure}
\begin{figure}[!tb]
	\centering
	\includegraphics[width=0.75\textwidth]{figures/seq2}
	\caption{The same DNA sequences of \Cref{fig:seq1}
		with the implanted pattern ATGCAACT.}
	\label{fig:seq2}
\end{figure}
\begin{figure}[!tb]
	\centering
	\includegraphics[width=0.75\textwidth]{figures/seq3}
	\caption{Same as \Cref{fig:seq2} with the implanted
		pattern ATGCAACT randomly
		mutated in two positions.}
	\label{fig:seq3}
\end{figure}


\section{Alignment Matrix}
To formulate the motif finding problem we first need to define
what we mean by motif. As we saw in \Cref{fig:seq3} there may be
mismatch in some positions of the motifs.

\begin{figure}%[!tb]
	\centering
	\includegraphics[width=0.6\textwidth]{figures/sindex}
	\caption{Starting index of motifs in a DNA sequence .}
	\label{fig:sindex}
\end{figure}


Now consider a set of \textit{t} DNA sequences $ S_{1}, S_{2},\ldots,
S_{t} $. Each of which has \textit{n} nucleotides. We select one
position in each of these \textit{t} sequences, thus forming an array
$ s = (s_{1}, s_{2},\ldots,s_{t}) $, where $ 1 \leq s_{i} \leq n - l + 1$
\Cref{fig:sindex}.
Here \textit{l} is the length of the pattern. The superposition
of the \textit{l}-mers of \Cref{fig:seq3} is shown in \Cref{fig:superpose}.
Now taking the \textit{l}-mers starting at these positions
we can compile a \textit{alignment matrix}\index{Alignment Matrix}
of $ t × l $. The $ (i, j) $th element of the \textit{alignment matrix}
is the nucleotide at the $ s_{i} + j − 1 $th position in the
\textit{i}th sequence. Illustrations are shown in \Cref{fig:consensus}.


\begin{figure}%[!tb]
	\centering
	\includegraphics[width=1.0\textwidth]{figures/superpose}
	\caption{Superposition of the seven highlighted 8-mers from \Cref{fig:seq2}.}
	\label{fig:superpose}
\end{figure}
\begin{figure}%[!tb]
	\centering
	\includegraphics[width=0.7\textwidth]{figures/consensus}
	\caption{The alignment matrix, profile matrix and consensus
		string formed from the 8-mers starting at positions
		$ s = (8, 19, 3, 5, 31, 27, 15) $ in \Cref{fig:seq2}.}
	\label{fig:consensus}
\end{figure}



\section{Profile Matrix}
The \textit{profile matrix}\index{Profile Matrix} or profile, illustrates
the variability of nucleotide composition at each position for
a particular group of \textit{l}-mers. Let the alphabet $ \Sigma $
in our motif search. Then the size of the \textit{profile matrix} will be
$ | \Sigma | \times l$. For DNA $ | \Sigma | = 4$.  Based on the
\textit{alignment matrix}, we can compute the $ 4 \times l $
\textit{profile matrix} whose $ (i, j) $th element holds the
number of times nucleotide $ i $ appears in column
$ j $ of the \textit{alignment matrix}, where $ i $ varies from 1 to 4.
In \Cref{fig:consensus} we see that positions 3, 7, and
8 are highly conserved, while position 4 is not.


\section{Consensus String}
To further summarize the profile matrix, we can form a consensus string from the most popular element in each column of the alignment matrix. It is the nucleotide with the largest entry in the profile matrix. \Cref{fig:consensus} shows the alignment matrix for s = (8,19,3,5,31,27,15), the corresponding profile matrix, and the resulting
consensus string ATGCAACT.

\section{Evaluating Motifs}
By varying the starting positions in s, we can construct a large number of
different profile matrices from a given sample. Some profiles represent high conservation of a pattern while others represent no conservation at all. An imprecise formulation of the Motif Finding problem is to find the starting positions s corresponding to the most conserved profile. 

\subsection{Scoring Function}
If $ P(s) $ denotes the profile matrix corresponding to starting positions s, then
we will use $ M_{P(s)}(j) $ to denote the largest count in column j of $ P(s) $. For
the profile P(s) in \Cref{fig:consensus}, $ M_{P(s)}(1) = 5, M_{P(s)}(2) = 5$ , and  $ M_{P(s)}(8) = 6 $.
Given starting positions s, the consensus score is defined to be $ Score(s, DNA) =
\sum_{j=1}^{l}M_{P(s)}(j) $. In our case, $ Score(s, DNA) =
5 + 5 + 6 + 4 + 5 + 5 + 6 + 6 = 42 $. $  Score(s, DNA) $ can be used to measure the strength of a profile corresponding to the starting positions s.


\section{Defining The Motif Finding Problem}
the Motif Finding problem can be formulated as selecting starting positions s from the sample that maximize $ Score(s, DNA) $. 
\begin{table}[H]
	\begin{center}
		\begin{tabular}{p{300 pt}}
			\hline
			\textbf{Motif Finding Problem:}\\
			\textit{Given a set of DNA sequences, find a set of l-mers, one from each
			sequence, that maximizes the consensus score.}\\
		
			\textbf{Input:} A t×n matrix of DNA, and l, the length of the pattern
			to find.\\
			
			\textbf{Output:} An array of t starting positions s = (s1, s2, . . . , st)
			maximizing Score(s, DNA).\\
			\hline
		\end{tabular}
	\end{center}
\end{table}

\endinput
